MASC: A Tool for Mutation-Based Evaluation of Static Crypto-API Misuse Detectors

While software engineers are optimistically adopting crypto-API misuse detectors (or crypto-detectors) in their software development cycles, this momentum must be accompanied by a rigorous understanding of crypto-detectors' effectiveness at finding crypto-API misuses in practice. This demo paper presents the technical details and usage scenarios of our tool, namely Mutation Analysis for evaluating Static Crypto-API misuse detectors (MASC). We developed $12$ generalizable, usage based mutation operators and three mutation scopes, namely Main Scope, Similarity Scope, and Exhaustive Scope, which can be used to expressively instantiate compilable variants of the crypto-API misuse cases. Using MASC, we evaluated nine major crypto-detectors, and discovered $19$ unique, undocumented flaws. We designed MASC to be configurable and user-friendly; a user can configure the parameters to change the nature of generated mutations. Furthermore, MASC comes with both Command Line Interface and Web-based front-end, making it practical for users of different levels of expertise.

==> masc-engine.tex <==
\begin{figure}[tbp]
    \centerline{\includegraphics[width=0.5\textwidth]{images/engine-status.png}}
    \caption{\small \tools{} Engine abstracts away details, and lets users download the compressed mutated application.}\label{fig:engine-status}
\end{figure}


==> masc-lab.tex <==
\begin{figure}[tbp]
    \centerline{\includegraphics[width=0.5\textwidth]{images/masc-lab.png}}
    \caption{\small \tools{} Lab portion lets users play with configurations to help them observe and learn about mutation and mutated crypto-API misuse cases}\label{fig:masc-lab}
\end{figure}

==> methodology.tex <==
\section{Methodology}
\label{sec:methodology}

==> restrictive.tex <==
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,float,numbers=none,caption={{\small
    \textit{Retrictive} crypto-API based mutant from \tool{}}},belowcaptionskip=-5mm,label=lst:restrictive,emph={mutation},emphstyle=\bfseries, language=java]
val = new Date(System.currentTimeMillis()).toString();
new IvParameterSpec(val.getBytes(),0,8);}
\end{lstlisting}

